Estimating the Level of Dialectness Predicts Interannotator Agreement in Multi-dialect Arabic Datasets

On annotating multi-dialect Arabic datasets, it is common to randomly assign the samples across a pool of native Arabic speakers. Recent analyses recommended routing dialectal samples to native speakers of their respective dialects to build higher-quality datasets. However, automatically identifying the dialect of samples is hard. Moreover, the pool of annotators who are native speakers of specific Arabic dialects might be scarce. Arabic Level of Dialectness (ALDi) was recently introduced as a quantitative variable that measures how sentences diverge from Standard Arabic. On randomly assigning samples to annotators, we hypothesize that samples of higher ALDi scores are harder to label especially if they are written in dialects that the annotators do not speak. We test this by analyzing the relation between ALDi scores and the annotators' agreement, on 15 public datasets having raw individual sample annotations for various sentence-classification tasks. We find strong evidence supporting our hypothesis for 11 of them. Consequently, we recommend prioritizing routing samples of high ALDi scores to native speakers of each sample's dialect, for which the dialect could be automatically identified at higher accuracies.

==> confidence-interval-plots.tex <==
\subsection{Confidence Interval Computation}
Apply bootstraping then split the data into two parts according to the ALDi scores and measure the difference in the agreement scores between the two groups!

The confidence interval for the mean difference in scores is computed using the values at the 2.5\% and 97.5\% percentiles of the data.

\todo[inline]{Fancier method \url{https://github.com/neshitov/bootstrap_interval}}

\begin{table*}
    \small
    \centering
    \begin{tabular}{llcl}
        \textbf{Label} & \textbf{Dataset} & \multicolumn{2}{c}{\textbf{Mean difference in full agreement percentages between low and high ALDi samples}}\\
        \midrule
        dialect & ArSarcasm-v1 & \drawnumberline{0.46}{5.2}{Purple} & $[0.46, 5.2]$ \\
        dialect & DART & \drawnumberline{-16.45}{-12.13}{Purple} & $[-16.45, -12.13]$ \\
        dialect & Arabic dialect familiarity & \drawnumberline{-16.43}{-8.48}{Purple} & $[-16.43, -8.48]$ \\
        \midrule
        hate speech & L-HSAB & \drawnumberline{4.85}{8.51}{Purple} & $[4.85, 8.51]$ \\
        hate speech & YouTube cyberbullying & \drawnumberline{5.73}{8.93}{Purple} & $[5.73, 8.93]$ \\
        misogyny general & LetMI & \drawnumberline{-0.2}{1.58}{orange} & $[-0.2, 1.58]$ \\
        misogyny specific & LetMI & \drawnumberline{5.52}{12.25}{Purple} & $[5.52, 12.25]$ \\
        offensive & DCD & \drawnumberline{-2.36}{0.69}{orange} & $[-2.36, 0.69]$ \\
        offensive & MPOLD & \drawnumberline{-5.68}{-0.74}{Purple} & $[-5.68, -0.74]$ \\
        \midrule
        qweet & qweet & \drawnumberline{-0.6}{4.92}{orange} & $[-0.6, 4.92]$ \\
        \midrule
        sarcasm & ArSarcasm-v1 & \drawnumberline{12.87}{17.05}{Purple} & $[12.87, 17.05]$ \\
        sarcasm & Mawqif sarcasm & \drawnumberline{15.19}{23.06}{Purple} & $[15.19, 23.06]$ \\
        sarcasm & arabic dialect familiarity & \drawnumberline{18.86}{26.64}{Purple} & $[18.86, 26.64]$ \\
        \midrule
        sentiment & ASAD & \drawnumberline{0.13}{4.95}{Purple} & $[0.13, 4.95]$ \\
        sentiment & ArSAS & \drawnumberline{1.75}{4.96}{Purple} & $[1.75, 4.96]$ \\
        sentiment & ArSarcasm-v1 & \drawnumberline{1.96}{7.48}{Purple} & $[1.96, 7.48]$ \\
        sentiment & Mawqif sarcasm & \drawnumberline{28.31}{37.79}{Purple} & $[28.31, 37.79]$ \\
        \midrule
        speech act & ArSAS & \drawnumberline{-4.15}{-0.89}{Purple} & $[-4.15, -0.89]$ \\
        \midrule
        stance & Mawqif stance & \drawnumberline{-0.1}{5.09}{orange} & $[-0.1, 5.09]$ \\
        \bottomrule
    \end{tabular}
    \caption{The confidence intervals (95\%) for the mean difference in full agreement proportions.}
\end{table*}

\begin{table*}
    \small
    \centering
    \begin{tabular}{llcl}
        \textbf{Label} & \textbf{Dataset} & \multicolumn{2}{c}{\textbf{Mean difference in full agreement all samples (low ALDi vs high ALDi)}}\\
        \midrule
        dialect & ArSarcasm-v1 & \drawnumberline{9.8}{14.55}{green} & $[9.8, 14.55]$ \\
        dialect & DART & \drawnumberline{-19.16}{-15.49}{green} & $[-19.16, -15.49]$ \\
        dialect & arabic dialect familiarity & \drawnumberline{-15.33}{-7.21}{green} & $[-15.33, -7.21]$ \\
        \midrule
        hate speech & L-HSAB & \drawnumberline{5.59}{10.07}{green} & $[5.59, 10.07]$ \\
        hate speech & YouTube cyberbullying & \drawnumberline{5.47}{8.27}{green} & $[5.47, 8.27]$ \\
        misogyny general & LetMI & \drawnumberline{-0.05}{1.67}{red} & $[-0.05, 1.67]$ \\
        misogyny specific & LetMI & \drawnumberline{5.25}{11.26}{green} & $[5.25, 11.26]$ \\
        offensive & DCD & \drawnumberline{-1.56}{1.34}{red} & $[-1.56, 1.34]$ \\
        offensive & MPOLD & \drawnumberline{-8.24}{-3.23}{green} & $[-8.24, -3.23]$ \\
        \midrule
        qweet & qweet & \drawnumberline{1.89}{6.98}{green} & $[1.89, 6.98]$ \\
        \midrule
        sarcasm & ArSarcasm-v1 & \drawnumberline{14.45}{18.68}{green} & $[14.45, 18.68]$ \\
        sarcasm & Mawqif sarcasm & \drawnumberline{17.22}{23.76}{green} & $[17.22, 23.76]$ \\
        sarcasm & arabic dialect familiarity & \drawnumberline{17.68}{27.23}{green} & $[17.68, 27.23]$ \\
        \midrule
        sentiment & ASAD & \drawnumberline{15.1}{16.23}{green} & $[15.1, 16.23]$ \\
        sentiment & ArSAS & \drawnumberline{0.79}{3.53}{green} & $[0.79, 3.53]$ \\
        sentiment & ArSarcasm-v1 & \drawnumberline{1.54}{5.09}{green} & $[1.54, 5.09]$ \\
        sentiment & Mawqif sarcasm & \drawnumberline{33.37}{41.2}{green} & $[33.37, 41.2]$ \\
        \midrule
        speech act & ArSAS & \drawnumberline{-4.3}{-0.94}{green} & $[-4.3, -0.94]$ \\
        \midrule
        stance & Mawqif stance & \drawnumberline{-0.2}{3.67}{red} & $[-0.2, 3.67]$ \\
        \end{tabular}
    \caption{The confidence intervals (95\%) for the mean difference in full agreement proportions.}
\end{table*}

% \begin{table*}
%     \small
%     \centering
%     \begin{tabular}{llcl}
%         \textbf{Label} & \textbf{Dataset} & \multicolumn{2}{c}{\textbf{Mean difference in full agreement percentages between MSA and DA samples}}\\
%         \midrule
%         dialect & ArSarcasm-v1 & \drawnumberline{11.27}{15.13}{green} & $[11.27, 15.13]$ \\
%         dialect & DART & \drawnumberline{-14.36}{-8.24}{green} & $[-14.36, -8.24]$ \\
%         dialect & arabic dialect familiarity & \drawnumberline{-2.62}{14.69}{red} & $[-2.62, 14.69]$ \\
%         \midrule
%         hate speech & L-HSAB & \drawnumberline{6.76}{12.62}{green} & $[6.76, 12.62]$ \\
%         hate speech & YouTube cyberbullying & \drawnumberline{-6.22}{0.38}{red} & $[-6.22, 0.38]$ \\
%         misogyny general & LetMI & \drawnumberline{-0.57}{1.35}{red} & $[-0.57, 1.35]$ \\
%         misogyny specific & LetMI & \drawnumberline{-8.44}{1.92}{red} & $[-8.44, 1.92]$ \\
%         offensive & DCD & \drawnumberline{0.9}{2.91}{green} & $[0.9, 2.91]$ \\
%         offensive & MPOLD & \drawnumberline{-8.61}{-2.03}{green} & $[-8.61, -2.03]$ \\
%         \midrule
%         qweet & qweet & \drawnumberline{5.84}{14.14}{green} & $[5.84, 14.14]$ \\
%         \midrule
%         sarcasm & ArSarcasm-v1 & \drawnumberline{7.28}{10.39}{green} & $[7.28, 10.39]$ \\
%         sarcasm & Mawqif sarcasm & \drawnumberline{6.84}{10.73}{green} & $[6.84, 10.73]$ \\
%         sarcasm & arabic dialect familiarity & \drawnumberline{7.32}{22.98}{green} & $[7.32, 22.98]$ \\
%         \midrule
%         sentiment & ASAD & \drawnumberline{13.13}{14.07}{green} & $[13.13, 14.07]$ \\
%         sentiment & ArSAS & \drawnumberline{-2.98}{-0.1}{green} & $[-2.98, -0.1]$ \\
%         sentiment & ArSarcasm-v1 & \drawnumberline{-1.14}{2.83}{red} & $[-1.14, 2.83]$ \\
%         sentiment & Mawqif sarcasm & \drawnumberline{13.09}{18.93}{green} & $[13.09, 18.93]$ \\
%         \midrule
%         speech act & ArSAS & \drawnumberline{-3.23}{-0.38}{green} & $[-3.23, -0.38]$ \\
%         \midrule
%         stance & Mawqif stance & \drawnumberline{-1.22}{1.35}{red} & $[-1.22, 1.35]$ \\
%     \end{tabular}
%     \caption{The confidence intervals (95\%) for the mean difference in full agreement proportions.}
% \end{table*}

% \begin{table*}
%     \small
%     \centering
%     \begin{tabular}{llcl}
%         \textbf{Label} & \textbf{Dataset} & \multicolumn{2}{c}{\textbf{Mean difference in full agreement percentages between low and high ALDi samples}}\\
%         \midrule
%         dialect & ArSarcasm-v1 & \drawnumberline{-0.03}{5.7}{orange} & $[-0.03, 5.7]$ \\
%         dialect & DART & \drawnumberline{-17.31}{-12.66}{Purple} & $[-17.31, -12.66]$ \\
%         dialect & arabic dialect familiarity & \drawnumberline{-16.68}{-8.44}{Purple} & $[-16.68, -8.44]$ \\
%         \midrule
%         hate speech & L-HSAB & \drawnumberline{3.79}{8.85}{Purple} & $[3.79, 8.85]$ \\
%         hate speech & YouTube cyberbullying & \drawnumberline{5.65}{8.89}{Purple} & $[5.65, 8.89]$ \\
%         misogyny general & LetMI & \drawnumberline{-0.11}{1.64}{orange} & $[-0.11, 1.64]$ \\
%         misogyny specific & LetMI & \drawnumberline{6.11}{12.74}{Purple} & $[6.11, 12.74]$ \\
%         offensive & DCD & \drawnumberline{-2.44}{1.22}{orange} & $[-2.44, 1.22]$ \\
%         offensive & MPOLD & \drawnumberline{-6.47}{-0.64}{Purple} & $[-6.47, -0.64]$ \\
%         \midrule
%         qweet & qweet & \drawnumberline{-0.27}{5.05}{orange} & $[-0.27, 5.05]$ \\
%         \midrule
%         sarcasm & ArSarcasm-v1 & \drawnumberline{12.55}{18.14}{Purple} & $[12.55, 18.14]$ \\
%         sarcasm & Mawqif sarcasm & \drawnumberline{14.5}{22.72}{Purple} & $[14.5, 22.72]$ \\
%         sarcasm & arabic dialect familiarity & \drawnumberline{17.16}{27.68}{Purple} & $[17.16, 27.68]$ \\
%         \midrule
%         sentiment & ASAD & \drawnumberline{11.19}{12.66}{Purple} & $[11.19, 12.66]$ \\
%         sentiment & ArSAS & \drawnumberline{1.48}{5.24}{Purple} & $[1.48, 5.24]$ \\
%         sentiment & ArSarcasm-v1 & \drawnumberline{1.37}{7.22}{Purple} & $[1.37, 7.22]$ \\
%         sentiment & Mawqif sarcasm & \drawnumberline{28.3}{39.61}{Purple} & $[28.3, 39.61]$ \\
%         \midrule
%         speech act & ArSAS & \drawnumberline{-4.56}{-1.15}{Purple} & $[-4.56, -1.15]$ \\
%         \midrule
%         stance & Mawqif stance & \drawnumberline{0.06}{4.43}{Purple} & $[0.06, 4.43]$ \\
%         \bottomrule
%     \end{tabular}
%     \caption{The confidence intervals (95\%) for the mean difference in full agreement proportions.}
% \end{table*}

\begin{figure*}
    \includegraphics[width=0.35\textwidth]{pre-bug-plots/heatmap.pdf}
\end{figure*}


==> histograms.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[]{plots/ArSAS_10_ALDi.pdf}
        \caption{ArSAS}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[]{plots/DART_10_ALDi.pdf}
        \caption{DART}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[]{plots/DCD_10_ALDi.pdf}
        \caption{DCD}
    \end{subfigure}%
    \vfill
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[]{plots/ArSarcasm-v1_10_ALDi.pdf}
        \caption{ArSarcasm-v1}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[]{plots/YouTube_cyberbullying_10_ALDi.pdf}
        \caption{YouTube Cyberbullying}
    \end{subfigure}%
    \vfill
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[]{plots/Mawqif_stance_10_ALDi.pdf}
        \caption{Mawqif (Stance)}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[]{plots/MPOLD_10_ALDi.pdf}
        \caption{MPOLD}
    \end{subfigure}
    \vfill
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[]{plots/arabic_dialect_familiarity_10_ALDi.pdf}
        \caption{Arabic Dialect Familiarity}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[]{plots/LetMI_10_ALDi.pdf}
        \caption{LetMI}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        \includegraphics[]{plots/qweet_10_ALDi.pdf}
        \caption{Qweet}
    \end{subfigure}%

    \caption{Histograms of the ALDi scores across the analyzed datasets.}
\end{figure*}


==> trends.tex <==
\begin{figure*}[t!]
    \centering
    \scriptsize{\textbf{Sentiment Analysis}}\\
    \begin{flushleft}
        \vspace{-0.65cm}
        \rule{16.5cm}{0.1mm}
        \vspace{-0.48cm}
    \end{flushleft}

    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[]{plots/ArSAS_10_sentiment_merged.pdf}
        % \caption{ArSAS}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[]{plots/ArSarcasm-v1_10_sentiment_merged.pdf}
        % \caption{ArSarcasm-v1}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[]{plots/ASAD_10_sentiment_merged.pdf}
        % \caption{ArSarcasm-v1}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[]{plots/Mawqif_sarcasm_10_sentiment_merged.pdf}
        % \caption{Mawqif}
    \end{subfigure}%
    \vfill
    
    \scriptsize{\textbf{Sarcasm Detection}}\\
    \begin{flushleft}
        \vspace{-0.4cm}
        \rule{12cm}{0.1mm}
        % \vspace{-0.48cm}
    \end{flushleft}

    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[]{plots/arabic_dialect_familiarity_10_sarcasm_merged.pdf}
        % \caption{Arabic Dialect Familiarity}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[]{plots/ArSarcasm-v1_10_sarcasm_merged.pdf}
        % \caption{ArSarcasm-v1}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[]{plots/Mawqif_sarcasm_10_sarcasm_merged.pdf}
        % \caption{Mawqif}
    \end{subfigure}%
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \vspace{-3cm}
        \scriptsize{\underline{\textbf{Speech Act Detection}}}
        \includegraphics[]{plots/ArSAS_10_speech_act_merged.pdf}
        % \caption{ArSAS}
    \end{subfigure}%
    \vfill

    \scriptsize{\underline{\textbf{Offensive Text Classification and Hate Speech Detection}}}
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[]{plots/MPOLD_10_offensive_merged.pdf}
        % \caption{MPOLD}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[]{plots/DCD_10_offensive_merged.pdf}
        % \caption{DCD}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[]{plots/YouTube_cyberbullying_10_hate_speech_merged.pdf}
        % \caption{YouTube Cyberbullying}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \vspace{-2.75cm}
        \scriptsize{\underline{\textbf{Stance Detection}}}
        \includegraphics[]{plots/Mawqif_stance_10_stance_merged.pdf}
        % \caption{Mawqif}
    \end{subfigure}%
    \vfill
    
    \scriptsize{\underline{\textbf{Arabic Dialect Identification}}}

    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[]{plots/arabic_dialect_familiarity_10_dialect_merged.pdf}
        % \caption{Arabic Dialect Familiarity}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[]{plots/ArSarcasm-v1_10_dialect_merged.pdf}
        % \caption{ArSarcasm-v1}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[]{plots/DART_10_dialect_merged.pdf}
        % \caption{DART}
    \end{subfigure}%
    % ~
    % \begin{subfigure}[t]{0.25\textwidth}
    %     \centering
    %     \vspace{-2.75cm}
    %     \scriptsize{\underline{\textbf{Answer-seeking Question Identification}}}
    %     \includegraphics[]{plots/qweet_10_qweet_merged.pdf}
    %     % \caption{Qweet}
    % \end{subfigure}%

    \caption{A scatter plot showing the relationship between binned ALDi scores (x-axis) and the percentage of samples with full agreement annotations (y-axis). The underlying histogram represents the number of samples per bin.}
    \label{fig:agreement_percentages}
\end{figure*}

